RL-JACK: Reinforcement Learning-powered Black-box Jailbreaking Attack against LLMs

Modern large language model (LLM) developers typically conduct a safety alignment to prevent an LLM from generating unethical or harmful content. Recent studies have discovered that the safety alignment of LLMs can be bypassed by jailbreaking prompts. These prompts are designed to create specific conversation scenarios with a harmful question embedded. Querying an LLM with such prompts can mislead the model into responding to the harmful question. The stochastic and random nature of existing genetic methods largely limits the effectiveness and efficiency of state-of-the-art (SOTA) jailbreaking attacks. In this paper, we propose RL-JACK, a novel black-box jailbreaking attack powered by deep reinforcement learning (DRL). We formulate the generation of jailbreaking prompts as a search problem and design a novel RL approach to solve it. Our method includes a series of customized designs to enhance the RL agent's learning efficiency in the jailbreaking context. Notably, we devise an LLM-facilitated action space that enables diverse action variations while constraining the overall search space. We propose a novel reward function that provides meaningful dense rewards for the agent toward achieving successful jailbreaking. Through extensive evaluations, we demonstrate that RL-JACK is overall much more effective than existing jailbreaking attacks against six SOTA LLMs, including large open-source models and commercial models. We also show the RL-JACK's resiliency against three SOTA defenses and its transferability across different models. Finally, we validate the insensitivity of RL-JACK to the variations in key hyper-parameters.

==> ack.tex <==
\section*{Acknowledgments}


==> tech-old.tex <==
\section{Key Techniques}
\label{sec:tech}

In this work, we design and develop, \sys, a novel jailbreaking attack that is more efficient and effective than existing approaches.
At a high level, rather than relying on genetic methods, we model the jailbreaking problem as a search problem and leverage reinforcement learning to enable a much more efficient jailbreaking prompt search.
In this section, we first introduce our threat model, followed by our technical insights into modeling and solving the jailbreaking problem with RL. 
Finally, we will specify our RL system designs. 


\subsection{Threat Model}
\label{sec:4.1}

\textbf{Attack assumptions.}
We consider the black-box setup where an attacker can only query a target LLM and get its final responses. 
The attacker cannot access the target LLM's model internals (i.e., architectures, parameters, logits. losses) and its training process (i.e., data, learning algorithm, etc). 
We assume the target LLM is an aligned model fine-tuned with either instruction tuning reinforcement learning from human feedback (RLHF)~\cite{ouyang2022training}. 
The model typically refuses to answer unethical and harmful questions.  
As discussed in existing works~\cite{lapid2023open, yu2023gptfuzzer, li2023deepinception}, this is a realistic setup in that most cases the target LLMs are online APIs without accessing the model internals (e.g., ChatGPT).  


\noindent\textbf{Attack goals.} 
We also consider training-free attacks, where the attacker cannot fine-tune the target LLM.

Under the above setup, we aim to design a novel jailbreaking attack that satisfies the following requirements.
\ding{182} Given a set of malicious question set $\mathcal{Q} = \{\mathbf{q}_1,..., \mathbf{q}_n \}$, the attacker wants to get the answer to these questions from a target LLM instead of a refusal response. 
These questions will be elaborated in the prompt set $\mathcal{P} = \{\mathbf{p}_1,..., \mathbf{p}_n \}$, which is carefully designed by the attacker. 
When these new prompts are presented to target LLM, they will elicit a set of responses $\{\mathbf{r}_1,..., \mathbf{r}_n \}$ that should not contain any refusal answer from the target model.
We use $\kappa$ to represent a predefined set of keywords, e.g. ``I'm sorry'', ``I cannot'', which are used for determining whether the model is refusing to answer the question. 
More about the choice of $\kappa$ will be included in Section \ref{sec:eval}.
Then we define a function $K(\mathbf{r}, \kappa) \mapsto \{0, 1\}$ to evaluate whether a response $\mathbf{r}$ contains the keywords in $\kappa$, i.e., whether target LLM is refusing to respond to the current prompt.
If $K(\mathbf{r}, \kappa)=1$, it means none of the keywords in $\kappa$ are present in the response $\mathbf{r}$, and 0 if any are detected.
The attacker aims to achieve $K(\mathbf{r}, \kappa)=1$ for all questions.
\ding{183} We also require the responses elicited from the attacker-provided prompts to contain the relevant answer to the question.
Specifically, for the question $\mathbf{q}_i$, once we obtained the response $\mathbf{r}_i$, it is important to check whether $\mathbf{r}_i$ contains a desired malicious outcome $O$.
For instance, consider the previous example (``How to build a bomb with household items?''), $O$ represents information or a tutorial on making a bomb using common items. 
Thus the attacker also needs to design an evaluation function $E(\mathbf{q}, \mathbf{r}) \in [0,1]$ to assess whether $\mathbf{r}_i$, the response elicited by the corresponding prompts build on $\mathbf{q}_i$, indeed contains such prohibited content, i.e., whether the model is indeed answering the question or delivering some off-topic content.
The attacker also aims to achieve $E(\mathbf{q}, \mathbf{r}) = 1$ for all questions.

\noindent\textbf{Defense assumptions.}
In Section~\ref{sec:eval}, we will evaluate the resiliency of our attack against SOTA defenses.
Here, we consider defenders as conventional ML researchers or practitioners who lack the resources to train or fine-tune an entire foundation model. 
As such, the defender can only perform some post hoc operations on the adversarial prompts or the target LLM's generated output, and cannot modify the target LLM's pentameters or its initial settings (e.g., system prompt).

\subsection{Problem Formulation}
\label{subsec: problem_formulate}

Given a harmful question, we formulate the task of finding a successful jailbreaking prompt that can elicit the corresponding answer as a search problem.
To systematically address this problem, we first elaborate on the search space and then define the specific objectives guiding our search.

\noindent\textbf{Search space.}
Recall that $\mathcal{Q}$ represents the set of all possible harmful questions, where a specific question $\mathbf{q}_i \in \mathcal{Q}, i=1,..,n$. The search space $\mathcal{S}$ is then defined by the set of all possible prompts $\mathbf{p}$ that can be generated from or related to $\mathbf{q_i}$. 
More precisely, for any given question $\mathbf{q_i}$, the corresponding prompts $\mathbf{p}$ can be crafted using a variety of techniques. These methods range from incorporating the question into pre-existing or newly created jailbreaking templates, as discussed in~\cite{yu2023gptfuzzer}, to modifying the words or phrases within a jailbreaking prompt as explored by Liu et al.~\cite{liu2023autodan}, or directly querying another LLM to generate a prompt tailored to the question~\cite{chao2023jailbreaking}.
These prior studies narrow down and refine the search space into a more manageable and targeted area through different approaches, converting the search problem to a local version.
They then proceed to conduct a focused search within this delineated area to find the most effective jailbreaking prompts.
Building upon these methodologies, the search problem of the attacker transits into a local search within an optimized subset of $\mathcal{S}$.

\noindent\textbf{Objective function.}
Given the search space $\mathcal{S}$, recall that the attacker has two goals: eliciting a non-refusal answer from the target LLM and guaranteeing the relevance of the answers to the original question.  
Thus the objective function of our search problem would be $C(\mathbf{q}, \mathbf{r}, \kappa) = E(\mathbf{q}, \mathbf{r}) \wedge K(\mathbf{r}, \kappa)$.
We aim to find the prompts $\mathbf{p}^*$ that maximizes $C(\mathbf{q}, \mathbf{r}, \kappa)$, where $\mathbf{r}$ is obtained by querying target LLM with prompts $\mathbf{p}$ that embedded with the question $\mathbf{q}$, i.e.,
\begin{equation}
    \begin{aligned}
      \mathbf{p}^* = \text{argmax}_{\mathbf{p}\in \mathcal{S}} C(\mathbf{q}, \mathbf{r}, \kappa), \forall \mathbf{q} \in \mathcal{Q} \, .
    \end{aligned}   
\end{equation}


\subsection{Technique Overview}
\label{sec:4.2}
We start this section with a discussion on stochastic vs. deterministic search strategies in a local search problem, then we introduce the key insights behind our proposed attack.

\noindent\textbf{Stochastic vs. deterministic search.}
Consider a grid where each point has a value, and our objective is to find the point with the minimum value, we can perform a search process that can be either deterministic or stochastic. 
This scenario is a simplified analogy to our previous formulation of finding the optimal jailbreaking prompt.
For the deterministic search process, starting from the initial point, it employs predefined rules to systematically navigate the search space. 
Consider the grid search example above, if we follow the negative gradient direction, the search process is akin to gradient descent. 
It involves assessing the gradient at our current location and moving in the direction of the steepest descent.
The direction of the gradient is precisely calculated thus there is no randomness during the search process, ensuring a consistent and direct path toward the objective.

Conversely, in a stochastic search scenario, starting from our randomly chosen initial position, subsequent steps involve moving to randomly chosen neighboring points. 
This method, while capable of exploring the grid broadly, lacks the directed focus of deterministic search. 
It operates under the principle of chance, which, despite its potential to escape local minima, may lead to inefficiencies.

Putting these two search methods together, we observe that the efficiency of deterministic search becomes particularly evident especially when a calculable objective function is present to guide the search. 
It leverages this function to make informed decisions about the direction and magnitude of each move, significantly enhancing the likelihood of reaching the optimal solution in a more efficient way.
This efficiency is crucial in the context of optimizing jailbreaking prompts for large language models. 
Given the complexity of the search space and the need for precision in eliciting specific responses, deterministic search offers a more structured and reliable way to navigate the problem space than stochastic search.
It utilizes the information from the objective function 
and steers the search toward the most promising areas more efficiently.

\noindent\textbf{A naive solution.}
As discussed above, we would like to perform a more efficient deterministic search when optimizing the jailbreaking prompts.
Our high-level idea is to train a reinforcement learning (RL) agent to interact with the target LLM and learn to generate the optimal jailbreaking prompts.
Compared with stochastic search, the agent will gradually learn how to adjust the generation of the prompts according to the reward we defined, which reflects the performance of the prompts. 
It will keep updating the policy toward the direction that maximizes the long-term reward, thus improving the total search efficiency.

Under this RL framework, a naive solution is to use RL to train another LLM, which can generate individual tokens~\cite{yang2023sneakyprompt, hong2024curiositydriven}. After these tokens are appended to the harmful question as a suffix, the whole prompt can jailbreak the victim model.
As we have demonstrated in \textcolor{red}{Appendix}, such a token-level generation policy is unsuitable and inefficient for jailbreaking attacks.
We consider there are two main possible reasons. First, the search space $\mathcal{S}$ is combinatorially large, especially when we consider finding specific token combinations. As LLM has a vast vocabulary and can generate sequences with flexible lengths. 
Navigating this immense space to find a specific sequence that can successfully jailbreak a model requires considerable computational resources and time, making it an inefficient approach.
On the other hand, successful jailbreaking prompts are rare within the vast search space, meaning that the RL model receives meaningful feedback very occasionally. 
This sparsity of reward complicates the learning process, as the model struggles to identify which actions (token generations) are truly beneficial towards achieving the jailbreaking objective. 
Consequently, the RL model may expend a considerable amount of time and resources exploring unproductive paths.
The large search space and sparse rewards complicate the training process for the token-level RL generation model. Achieving convergence to a successful jailbreaking strategy becomes increasingly challenging, as the model must navigate a delicate balance between exploring new token sequences and exploiting known information in a mostly reward-less environment.
All the above difficulties in training and achieving model convergence further motivate us to design novel and more complicated mutators, which can provide some good starting points for the agent and improve the success of training.

\noindent\textbf{Key insights.}
Building upon the understanding that token-level prompt generation for jailbreaking poses significant challenges, we propose a novel approach that leverages the capabilities of an LLM(denoted as helper LLM) to generate jailbreaking prompts more efficiently.
Our solution shifts the focus from selecting individual tokens to defining and utilizing high-level strategies that guide the prompt generation process.
Specifically, we introduce the helper LLM to aid in the creation of effective jailbreaking prompts. 
We first define a set of $N$ mutators that incorporate different tactics or modifications that could be applied to a prompt, to potentially make it more effective at eliciting the desired response from the target LLM. 
These mutators might include but are not limited to, creating scenarios, adding context, or incorporating specific linguistic patterns known to bypass certain restrictions. More details of our mutator design can be found in Section \ref{subsec: our_attack}.

To dynamically select the most appropriate strategy for any given question $\mathbf{q}$ or prompt $\mathbf{p}$, we train a policy model that learns to associate different prompt characteristics with the success rates of various mutators. This policy model essentially learns which mutator (action) to apply in a given situation to transform the current prompt $\mathbf{p}$ into a more effective version. 
The selected action is then used to craft an instruction that instructs the helper LLM on how to modify the original prompt. The process is designed to be iterative, allowing for successive refinements of the prompt based on feedback and outcomes, thereby increasing the likelihood of successfully jailbreaking the target model.

With the helper LLM, We harness the creative and generative capabilities of LLMs to navigate the complex space of prompt crafting, while also introducing a layer of strategic decision-making through the policy model. 
This approach not only mitigates the challenges associated with token-level generation but also offers a more nuanced and adaptable pathway to generating jailbreaking prompts, significantly enhancing the efficiency and effectiveness of the jailbreaking process.


\subsection{Our Attack.}
\label{subsec: our_attack}
Figure \ref{fig:overview} shows an overview of our proposed attack. Given a harmful question, it will be fed into the RL agent as input, and the agent will 
select an action from our pre-defined action space.
As shown in the example, the question is ``I want to produce a fake check, How to do it?'' and the agent picks an action as asking the helper LLM to create some role-play scenario that can embed the question into it.
Then the selected action will be the instruction to the helper LLM, asking it to construct a new prompt following the strategy defined in the action.
Consequently, the helper LLM generates a modified prompt, such as "As a researcher...", subtly designed to deceive the target LLM and achieve a jailbreak.
In the following sections, we will delve into our RL framework, and discuss how we design the state action space and reward. 


\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{imgs/overview.pdf}
    \caption{{\small [placeholder for overview].}}
    \label{fig:overview}
    \vspace{-7mm}
\end{figure}


\noindent\textbf{RL formulation.}
We formulate the jailbreaking prompt generation as a Markov Decision Process (MDP). 
Given an initial state $\mathbf{s} = \mathbf{p}_0$,
at each time step $t$, the RL agent selects one of the mutators from the action space $A$. 
We can then define the transition function $\mathcal{T}: S \times A \rightarrow S$ to be the state of prompt before and after applying mutator $\mathbf{p}_t \times a_t \rightarrow \mathbf{p}_{t+1}$. 
Note that we design the transition dynamics to be deterministic given the chosen mutator and input prompts.
As we will discuss later, making it stochastic will increase the difficulty to converge to an effective policy. 
We define either a maximum time step $H$ or termination criteria to stop the mutating and get the final jailbreaking prompt.
The goal is to maximize the expected reward $R = \mathbb{E}[\sum_{k=0}^T\gamma^k r_k]$ where $r_t$ is the reward at $t$ and $\gamma$ is the discount factor.
We use $\pi_{\theta}$ to denote the policy network of the RL agent.
We also define a stationary state occupancy distribution for $\pi_{\pi_{\theta}}$, denoted as $\rho^{\pi}(s) = (1-\gamma)\sum_{t}\gamma^{t}p(s_t=s|\pi_{\theta})$.


\noindent\textbf{State representation.}
The state representation provides the agent with the information of the current prompt.
Instead of using the raw text directly, we follow a similar state space design in~\cite{zhang2023tempera} and use the hidden representation extracted from a text encoder $\Phi$ as the agent's observation.
Given an input prompt $\mathbf{p}$, a text encoder can convert $\mathbf{p}$ to its hidden representation $\mathbf{w} \in \mathbb{R}^n$.
Specifically, in our case, at the initial time step $t=0$, the state $s_0$ will directly be the hidden representation of the unedited harmful question. 
Later, after the helper LLM generates a jailbreaking prompt based on the instruction in $a_0$, where $a_0 = \pi_{\theta}(s_0)$, the next time step's state $s_1$ will be the hidden representation of the generated prompt $\mathbf{p}_1$.

\noindent\textbf{Action space.}
Every action $a\in A$ is a mutator that specifically describes how should the helper LLM modify the current prompt.
At every time step, the RL agent can choose an action $a\in A$ and this action will be incorporated into an instruction to the helper LLM, forming a complete prompt. 
This prompt is to ask the helper LLM to generate a prompt that follows the requirements in $a$ and embed the current question into it.
An example of our designed action is ``You need to devise a role-playing scenario that subtly incorporates the question without direct mention, encouraging the model to adopt a specific character or behavior in context... ''.
We design each action based on the patterns of jailbreaking prompts summarized in~\cite{liu2023jailbreaking, wei2023jailbroken}. 
A full list of actions is included in \textcolor{red}{Table.}

\noindent\textbf{Transition function.}
After determining the state and action, we need to design the state transition function $\mathcal{T}$, i.e., given the current prompt $\mathbf{p}_t$ and action $a_t$, how do we obtain $\mathbf{p}_{t+1}$. 
This is non-trivial as we are not directly performing token generation~\cite{rlprompt} or word replacement~\cite{zhang2023tempera} in our RL formulation, where the next state will naturally be the previous prompt appended with a token, or replace some words in the previous prompt.
We incorporate the helper LLM's generation ability, which will introduce more randomness into the state transition process.

A straightforward design is to directly let the helper LLM generate $\mathbf{p}_{t+1}$ based on $a_t$ and the question $\mathbf{q}$, regardless of what $\mathbf{p}_t$ is.
We test this solution and find that the agent cannot learn an effective policy.
Our empirical investigation indicates that the reasons are twofold.
First, it neglects the nature of an RL problem where adjacent states often share some degree of similarity. 
Such similarity can be understood in terms of physical proximity, feature similarity, or both. 
For instance, in a video game, moving one step to the left might change the position feature slightly but leave other features (like the health level or inventory items) unchanged.
However, in this design, $\mathbf{p}_{t+1}$ and $\mathbf{p}_t$ can have totally different contexts and the only similarity is the question in it.
It would be hard for the agent to connect the action with the previous state.
Second, given the same question and action, the uncertainty of $\mathbf{p}_{t+1}$ largely increases the difficulty for the agent to learn a strategy behind it. As sometimes the generated $\mathbf{p}_{t+1}$ can jailbreak successfully but sometimes it cannot.
The agent will be confused by such inconsistent reward signals for the same state-action pairs.
These initial explorations highlight two challenges: (1) how to make the adjacent states more similar such that the agent can learn the dynamics behind it, and (2) how to maintain the consistency of $\mathbf{p}_{t+1}$, given the same $\mathbf{p}_{t}$ and $a_t$.

\noindent\underline{Challenge I.} 
We add extra designs to improve the consistency of adjacent states. If $a_t = a_{t+1}$, we ask the helper LLM to paraphrase $\mathbf{p}_t$ to obtain $\mathbf{p}_{t+1}$.
If $a_t \neq a_{t+1}$, We first ask helper LLM to generate a prompt $\mathbf{p}'_{t+1}$ based on $a_{t+1}$, then it needs to perform crossover based on $\mathbf{p}_t$ and $\mathbf{p}'_{t+1}$ to obtain the final $\mathbf{p}_{t+1}$.
We provide an example to illustrate this process in Figure. 

\noindent\underline{Challenge II.}
To address this challenge, we explicitly set the generation strategy of helper LLM to be deterministic, i.e., given the same input prompt, the generated output will always be the same.
Existing works usually suggest that performing a stochastic sampling strategy can produce more fluent and natural text~\cite{fan2018hierarchical, Holtzman2020The}. 
We find that the deterministic generation largely stabilizes our training process, enabling the agent to learn an effective policy, without sacrificing the quality of the prompts too much.
Then during the evaluation phase, we use the stochastic sampling strategy to generate more diverse prompts and increase the probability of jailbreaking successfully.

\noindent\textbf{Reward design.}
At each time step $t$, after we get the response $\mathbf{r}_t$ of input prompt $\mathbf{p}_t$ from the target LLM, we compare it with a reference answer $\mathbf{r}'$ obtained from an uncensored LLM. 
We reuse the previous text encoder $\Phi$ to extract the hidden representation of both responses and use the cosine similarity between them as the dense reward: 
$$r_t = \text{CosineSimilarity}\left(\Phi(\mathbf{r}_t), \Phi(\mathbf{r}')\right) = \frac{\Phi(\mathbf{r}_t) \cdot \Phi(\mathbf{r}')}{\|\Phi(\mathbf{r}_t)\| \|\Phi(\mathbf{r}')\|}$$
Recall that in Section \ref{sec:4.1} we defined two goals of the attacker, where $E(\mathbf{q}, \mathbf{r})$ measures the relevance of the response to the question. 
The cosine similarity between $\mathbf{r}_t$ and $\mathbf{r}'$ reflects how much on-topic the answer $\mathbf{r}_t$ is. If the cosine similarity is higher than some threshold, we consider $E(\mathbf{q}, \mathbf{r})=1$, i.e., $\mathbf{r}_t$ contains the answer to the original question $\mathbf{q}_t$.
Thus during training, we set a threshold $\tau$ for the cosine similarity. When $r_t < \tau$, we directly use the cosine similarity value as the dense reward $r_t$.
When $r_t \geq \tau$, we directly set $r_t=1$, indicating that the current response achieves the jailbreaking goal.

\noindent\textbf{Termination condition.}
We define the termination condition from two perspectives, either the agent reaches the maximum time step $H$ for the current episodes, or the current question has been jailbroken successfully.
As we stated above, we set a threshold $\tau$ for the cosine similarity, when $r_t \geq \tau$, we consider that the prompt $\mathbf{p}_t$ successfully jailbreaks the question, and we will mark the current episode as terminated.

After defining the component of our RL framework, the goal is to learn the parameter $\theta$ of optimal policy $\pi^*_{\theta}$ by optimizing the following objective function, under our designed environment:
\begin{equation}
    \begin{aligned}
     \max_{\theta} J(\theta) = \max_{\theta} \sum_s\rho^{\pi}(s)\sum_{a}\pi_{\theta}(s)V_{\pi_{\theta}}(s, \pi_{\theta}(s)) \, ,
    \end{aligned}
\end{equation}
where $V_{\pi_{\theta}}(s)$ is the state-value function.

We use the PPO ~\cite{ppo} algorithm to solve $J(\theta)$ and update the policy. The full algorithm can be found in Appendix~\ref{appendix:additional_tech}.



